MWP-BERT: Numeracy-Augmented Pre-training for Math Word Problem Solving

Math word problem (MWP) solving faces a dilemma in number representation learning. In order to avoid the number representation issue and reduce the search space of feasible solutions, existing works striving for MWP solving usually replace real numbers with symbolic placeholders to focus on logic reasoning. However, different from common symbolic reasoning tasks like program synthesis and knowledge graph reasoning, MWP solving has extra requirements in numerical reasoning. In other words, instead of the number value itself, it is the reusable numerical property that matters more in numerical reasoning. Therefore, we argue that injecting numerical properties into symbolic placeholders with contextualized representation learning schema can provide a way out of the dilemma in the number representation issue here. In this work, we introduce this idea to the popular pre-training language model (PLM) techniques and build MWP-BERT, an effective contextual number representation PLM. We demonstrate the effectiveness of our MWP-BERT on MWP solving and several MWP-specific understanding tasks on both English and Chinese benchmarks.

==> table/old_probing.tex <==
\begin{table*}[t]
\small
\renewcommand\arraystretch{1.2}
\centering
\setlength{\tabcolsep}{0.95mm}{
\begin{tabular}{c|c|c|c|c|c|c|c}
\hline

            & s1 & s2 & w1 & w2 & w3 & f1 & f2   \\
\hline
BERT         & 3.08 & 0.87  & 0.75 & 0.77 & 0.77 & 0.97 & 0.50      \\
RoBERTa     & 3.20 & 0.86 & 0.76 & 0.78 & 0.77  & 0.99 & 0.51       \\
\hline
MWP-RoBERTa  & 0.69 & 0.92  & 0.86 & 0.87 & 0.86 & 0.44 & 0.86  \\
MWP-BERT  & 0.67 & 0.92  & 0.85 & 0.87 & 0.86 & 0.45 & 0.87 \\
\hline
\end{tabular}}
\caption{The evaluation on probing tasks. All tasks are described in our methodology section. Note that the metric for task s1 and f1 is mean-squared-error, while others use classification accuracy.}
\label{tab:result_probing}
\end{table*}

==> table/tab_mwp_result.tex <==
\begin{table*}[t]
\renewcommand\arraystretch{0.95}
\centering
\setlength{\tabcolsep}{0.8mm}{
\begin{tabular}{l|cc|cc|cc}
\hline
% \multicolumn{1}{c|}{\multirow{3}{*}{Model}} & \multicolumn{6}{c||}{Sentence Ordering} & \multicolumn{6}{c}{Image Ordering} \\ \cline{2-13} 
\multicolumn{1}{c|}{\multirow{2}{*}{\textbf{Model}}} & \multicolumn{2}{c|}{\textbf{$\mathrm{Math23k}$}} & \multicolumn{2}{c|}{\textbf{$\mathrm{Math23k^*}$}} & \multicolumn{2}{c}{MathQA}  \\ \cline{2-7}
\multicolumn{1}{c|}{} & Equ-Acc  &Ans-Acc  & Equ-Acc  &Ans-Acc & Equ-Acc  &Ans-Acc  \\ \hline
    DNS              & - & - & - & 58.1 & - & -   \\
    Math-EN          & 60.1 & 66.7 & - & - & - & -   \\
    GTS              & - & 75.6 & - & 74.3 & - & 71.3  \\
    NS-Solver        & - & 75.7 & - & - & - & -   \\
    Graph2Tree       & 66.2 & 77.4 & 62.1 & 75.5 & 70.0 & 72.0   \\
    TSN-MD           & 65.8 & 77.4 & - & 75.1 & - & -   \\
    KA-S2T           & - & 76.3 & - & - & - & -   \\
    NumS2T           & - & 78.1 & - & - & - & -   \\
    EEH-G2T          & - & 78.5 & - & - & - & -   \\
\hline
    RPKHS            & - & 83.9 & - & 82.2 & - & -   \\
 \hline
  \textbf{Encoder Pre-trianing}            &  &  &  &  &  &    \\
    \quad RoBERTa          & $71.1$ & $83.5$ & $70.6$ &  $81.7$ & $73.8$ & $75.3$   \\
    \quad BERT             & $71.7$ & $83.8$  & $70.7$ & $82.0$ & $73.6$ & $75.1$   \\
    \quad MWP-RoBERTa (Ours)      & $71.9$ & ${84.5}$ & $\mathbf{71.2}$ & ${82.0}$  & $\mathbf{74.9}$ & $\mathbf{76.6}$  \\
    \quad MWP-BERT (Ours)        & $\mathbf{72.0}$ & $\mathbf{84.7}$ & $71.0$ & $\mathbf{82.4}$ & $74.1$ & $76.2$   \\
\hline \hline
      \textbf{Seq2Seq Pre-trianing}            &  &  &  &  &  &    \\
\quad REAL             & - & 82.3 & - & 80.0 & - & -   \\
\quad BERT-CL          & 71.8 & 83.2 & - & - & 74.4 & 76.3  \\
\quad Gen\&Rank      & - & 85.4 & - & 84.3 & - & -   \\
\hline
\end{tabular}
}
\caption{Comparison of answer accuracy (\%) between our proposed models and different baselines on Math23k and MathQA dataset, separated by the middle split line. $\mathrm{Math23k}$ column shows the results when evaluating on the public test set of Math23k. $\mathrm{Math23k^*}$ column shows the result of 5-fold cross validation on Math23k dataset. MathQA is adapated from~\citet{li2021seeking,DBLP:journals/corr/Tan2021multilingual}. ``RoBERTa'' and ``BERT'' represent results without pre-training. ``MWP-RoBERTa'' and ``MWP-BERT'' represent first pre-training with proposed techniques and then fine-tuning.}
\label{tab:main_result}
\end{table*}

==> table/table_intro_example.tex <==
\begin{table}[t]
\renewcommand\arraystretch{1.2}
\centering
\begin{tabular}{|m{1.8cm}<{\centering}|m{5.3cm}<{\centering}|}
\hline
Problem Description: & Some workers are producing 660 clothes. It has been 5 days and 75 clothes are produced per day. But they have to finish all clothes in 3 more days. How many clothes should be processed per day from now? \\ 
\hline
Value Solution:  &  x = 95  \\
\hline
Equation Solution: &  x = (660-75*5)/3 = 95 \\
\hline
\end{tabular}
\caption{This table shows an example of MWP. Most MWP solvers are trained under fully-supervised setting with the equation solution. In this paper, we design several pre-training tasks that enable the MWP solver learning from problem description (self-supervised), value solution (weakly-supervised) and equation solution (fully-supervised).
}
\label{tab:data_intro}
\end{table}

==> text/introduction1.tex <==
\section{Introduction}
\input{figure/fig_intro}
Recent works in math word problem (MWP) solving~\cite{wang2018translating,wang2019template,liu2019tree,li2019modeling,xie2019goal,zhang2020graph,DBLP:conf/acl/WuZWH20,DBLP:conf/acl/QinLHTL20,DBLP:conf/emnlp/HuangWXCY21,DBLP:conf/emnlp/WuZW21,DBLP:conf/emnlp/YuWZX21,DBLP:conf/emnlp/ShenYLSJ0021} arrange  the  pipeline into a sequence-to-sequence framework. In brief, they use deep representation and gradient optimization as well as symbolic constraints to discover discrete symbolic combination of operators and variants. Fundamentally, MWP solving system aims to perform symbolic reasoning by searching through a combinatorial solution space given the text description evidences. Thus, 
these neurosymbolic methods mainly focus on getting more effective semantic representations~\cite{li2019modeling,zhang2020graph,DBLP:conf/acl/WuZWH20,DBLP:conf/emnlp/WuZW21,DBLP:conf/emnlp/YuWZX21}, injecting symbolic constraints~\cite{wang2018translating,wang2019template,liu2019tree,xie2019goal} and how to align semantic space (text descriptions) and huge combinatorial symbolic space (symbolic solutions)~\cite{DBLP:conf/acl/QinLHTL20,DBLP:conf/emnlp/ShenYLSJ0021,DBLP:conf/emnlp/HuangWXCY21}. This line of methods has achieved great success and is still holding the lead in various MWP solving benchmarks~\cite{wang2017deep,zhao2020ape210k,koncel2016mawps}. 
%Fundamentally, we can identify two challenges for this neurosymbolic pipeline. First, MWP solving system must perform symbolic reasoning by searching through a combinatorial and quickly exploding solution space. More exactly, there exists mismatch between semantic space (text descriptions) and huge combinatorial symbolic space (symbolic solutions). It is difficult to align between text tokens appeared once in problem descriptions and repeatedly appeared symbols in solution. Second, what is even worse is that 

Despite the great performance achieved by the previous methods, there still exists fundamental challenges in number representation for MWP solving. More exactly, number values are required to be considered as vital evidence in solution exploration but existing works are known to be inefficient in capturing numeracy information~\cite{DBLP:conf/emnlp/WallaceWLSG19}. Intuitively, we could simply treat explicit numbers in the same way with words, i.e., assign position for all numbers in the vocabulary. However, there would be infinite number of candidates during prediction and it would be impossible to learn their deep representations. In other words, the solution space will be extremely large and the complexity is unacceptable. Therefore, almost all existing works follow ~\citet{wang2017deep} to replace all numbers with symbolic placeholders (e.g., ``x1'', ``x2''). The core idea here is to get a reasonable solution space by restricting neural networks to leave out numerical characteristics and focus on logic reasoning. However, this method will transform the number representation learning as a two-level ill-conditioned problem. Firstly, number representation naturally faces severe polysemy issues even without substitution. Compared with word representations, meanings of numbers will vary quite a lot in different text descriptions, e.g., ``100'' in ``Each desk is worth \$ 100 '' is totally different from that in ``move 100 packages''. Suppose there are $n$ MWP examples in a given  dataset, ``100'' will have $n$ meanings at worst case. This issue is termed as number polysemy in this work. Secondly, symbolic placeholders will introduce extra numerical polysemy issue here, i.e., ``x1'' can be any real number that appeared in the specific dataset. In general, ``x1'' can be any real number in the number field. We term this issue as symbol polysemy. When putting these two issues together, we can observe a compound number-symbol polysemy issue which will bring severe ambiguity issue for MWP understanding and solving.

For number polysemy, we propose to transform static (context-independent) word embeddings to dynamic (context-dependent) representations by pre-trained language model (PLM)~\cite{devlin2019bert,liu2019roberta}. Compared with traditional word embedding techniques which assign single prototype vector for each word, PLMs provide dynamic context-dependent representation to support grabbing polysemy  over contexts In detail, static word embedding usually assigns a single prototype vector for each word that does not change with context. It is naturally deficient in grabbing multiple meanings for single tokens. An effective way to resolve this issue is to introduce dynamic representations. In order to get contextual representations, the representation module is usually pre-trained on a large-scale corpus with self-supervised learning objectives to predict masked tokens by their context. These dynamic representations obtained can be easily plugged into various downstream tasks and consistently achieve great performance across various tasks~\cite{beltagy2019sciBERT,lee2020bioBERT,yang2020finbert}. 

For symbol polysemy, we incorporate several numeracy grounded pre-training objectives to inject inductive bias about numerical constraints into dynamic representations. Compared with word candidate sets, useful points in number candidate space is sparse. However, we identify that during prediction, what matters is reusable numerical properties of number values. What's more, these properties do not suffer from sparsity issues like number values. Therefore, compared with assigning a prototype vector for each single number value, it is more reasonable to inject the reusable numerical properties in deep representations, e.g., magnitude and number type. Here, since PLM is chosen as our backbone to get dynamic representations for numbers, we propose to design numeracy grounded pre-training objectives to implement soft constraints between symbolic placeholders and numbers in deep representation.

\textbf{Contributions.} We introduce a numeracy PLM, MWP-BERT to make encoders to better understand the numerical property in MWP solving. Besides, a group of numeracy grounded pre-training objectives is designed to leverage the corpus of MWP and encourage the contextual representation to capture numerical information. Experiments made on both Chinese and English benchmarks show significant improvement overall competitors. To our knowledge, this is the first approach that surpasses human performance \cite{wang2019template} in terms of MWP solving.
%[BERT is strong. Understanding ability, multi-modal input, symbolic understanding BERT]


==> text/old_abstract.tex <==
\begin{abstract}


%Math word problem (MWP) solving is the task of transforming a sequence of natural language problem descriptions to executable math equations.
%An MWP solver not only needs to perceive number properties like magnitudes, but also identify the key mathematical variables and associate text descriptions with mathematical logic. 
Pre-training language models (PLM) are known to be good at capturing semantic information via contextual modeling and distribution hypothesis. However, PLMs like BERT and RoBERTa have several flaws when adapting to Math word problem (MWP) solving: 1) They do not have built-in mathematical knowledge and fail to effectively grab numerical properties in the text; 2) Single numeracy-aware contextual modeling do not consider the discrepancy between numeracy understanding (encoding) and solution generation (decoding). This would lead to an extra requirement of human-annotated Question-Solution parallel corpus and hinder the broader application.
%Although recent sequence modeling MWP solvers have gained credits on the  math-text contextual understanding, pre-trained language models (PLM) have not been explored for solving MWP, considering that PLM trained over free-form texts is limited in representing text references to mathematical logic. 
In this work, we introduce MWP-BERT with a novel suite of methodology to learn effective contextual number representations. It contains 8 pre-training tasks to leverage unlabeled, incompletely labeled and fully labeled MWPs in scenarios of unsupervised, weakly supervised and fully supervised learning. 
%to obtain pre-trained token representations that capture the alignment between text description and mathematical logic. 
We demonstrate the effectiveness of our MWP-BERT on 2 different downstream tasks and 7 probing tasks. Moreover, MWP-BERT outperforms the strongest competitor by a large margin (5-10\% accuracy improvement) on the two largest MWP solving benchmarks. %Extensive ablations also demonstrate that the model gets improved from the proposed pre-training tasks. 



\end{abstract}

==> text/old_experiment.tex <==
\section{Experiments}

We present several empirical results in this section to prove the superiority of MWP-BERT. We firstly introduce our newly curated Ape-clean dataset. Then We give the MWP probing results to demonstrate the numerical understanding ability. Next, we evaluate MWP-BERT on MWP solving and quantity tagging~\cite{DBLP:conf/acl/ZouL19}. Finally, we present our ablation experiments.  

\subsection{The Ape-clean Dataset}
%\paragraph{Math23k.}
%Math23k \cite{wang2017deep} is a widely used dataset to evaluate MWP solvers. It contains 21,162 Chinese math word problems in the training set and 1000 problems in the test set. Evaluation results can be reported on test set, while  researchers also bind its training and test set together and perform 5-fold cross validation on this dataset. We report the results in both settings.
\input{table/tab_experiment_removed_cases}

%\paragraph{Ape-clean.}
Ape210k is a recently released large MWPs dataset, including 210,488 problems. 
The problems in Ape210k are more diverse and difficult than those in Math23k as shown in \ref{tab:data_demo}. Not only the stronger requirement of common-sense knowledge for getting solutions, but also the missing of ground-truth solution equations or answers, will take extra obstacles for MWP solving. Among all these cases, 
the problems without answers can not be used for fully-supervised setting. Besides, the problems without annotated equations but only answer values
can be used in the weakly-supervised learning setting. 
Therefore, we follow the rules below to select the usable problems from Ape210k to construct an Ape-clean dataset, which can be used for the fully-supervised learning setting. (i). We remove all MWPs that  have no answer values nor equations.
(ii). We remove all MWPs that only have answer values without equations. 
(iii). We remove all MWPs with a problem length $m > 100$ or an answer equation length $n > 20$, as they will bring obstacles for training. %We cannot perform truncation on over-length problems or answers because incomplete problems are unsolvable and incomplete answers are meaningless to work on.
(iv). We remove all MWPs requiring external constants except $1$ and $\pi$.
(v). We remove all duplicated problems with the MWPs in Math23k.
After data filtering, the \emph{Ape-clean} dataset contains 81,225 MWPs, including 79,388 training problems and 1,837 testing problems. The remaining 129,263 problems in Ape210k are regarded as \emph{Ape-unsolvable}, which can be used in the pre-training tasks in the settings of self-supervised and weakly-supervised learning.


%Although around half of problems in Ape210k are filtered out, the over 125K high-quality problems are sufficient to be used for MWP solving. Moreover, we leave the remaining dataset as Ape-unsolvable and present several pre-training tasks to utilize those problems. 

\subsection{Implementation Details}
We pre-train our model on 4 NVIDIA TESLA V100 graphic cards and fine-tune on 1 card. All implementation\footnote{We will release all the materials including code and data after this paper is accepted.} of training and testing is coded in Python with Pytorch framework. The model was pre-trained for 50 epochs and fine-tuned for 80 epochs with a batch size of 32. Adam optimizer \cite{kingma2014adam} is applied with an initial learning rate of 5e-5, which would be halved every 30 epochs. During testing, we use 5-beam search to get reasonable solutions. For the pre-trained model, we use an upgrade patch of Chinese BERT and RoBERTa which are pre-trained with the whole word masking (WWM) \footnote{\url{https://github.com/ymcui/Chinese-BERT-wwm}} \cite{cui2020revisiting}. The hyper-parameters setting of our BERT and RoBERTa is 12 layers of depth, 12 heads of attention and 768 dimensions of hidden features. 

\subsection{Probing Tasks}
Here, we investigate the impact of MWP-BERT in MWP understanding task by performing probing tasks. Probing not only aims to infuse knowledge into pre-trained models, but it can also evaluate PLMs as mentioned in \cite{DBLP:conf/acl/XuGTSSGZQJD20}. Note that evaluation is conducted in a zero-shot setting where the parameters of MWP-BERT are fixed and other parameters in feed-forward blocks are randomly initialized for the sake of fair comparison.

\begin{table}
\small
\renewcommand\arraystretch{1.2}
\centering
\setlength{\tabcolsep}{0.95mm}{
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline

            & s1 & s2 & w1 & w2 & w3 & f1 & f2   \\
\hline
BERT         & 3.08 & 0.87  & 0.75 & 0.77 & 0.77 & 0.97 & 0.50      \\
RoBERTa     & 3.20 & 0.86 & 0.76 & 0.78 & 0.77  & 0.99 & 0.51       \\
\hline
MWP-RoBERTa  & 0.69 & 0.92  & 0.86 & 0.87 & 0.86 & 0.44 & 0.86  \\
MWP-BERT  & 0.67 & 0.92  & 0.85 & 0.87 & 0.86 & 0.45 & 0.87 \\
\hline
\end{tabular}}
\caption{The evaluation on probing tasks. All tasks are described in our methodology section. Note that the metric for task s1 and f1 is mean-squared-error, while others use classification accuracy.}
\label{tab:result_probing}
\end{table}

Following the probing task design in \cite{DBLP:conf/naacl/HewittM19,DBLP:conf/emnlp/WallaceWLSG19}, we make the following probing tasks to test if the model learns effective representation:

We report the performances of BERT, RoBERTa, MWP-BERT and MWP-RoBERTa on the probing tasks in Table \ref{tab:result_probing}. The results demonstrate that our proposed pre-training does enhance the numerical understanding ability of PLMs. This group of probing tasks could also serve as a special evaluation setting for future MWP-related PLMs.



\subsection{MWP Solving}\label{experiment:mwpsolving}
\paragraph{Experiment Setting and Datasets.}
Given a textual description of a mathematical problem, which contains several known variables, MWP solving targets at getting the correct answer for the corresponding question. A solver is expected to be able to predict an equation which can exactly reach the answer value. MWP solving is the most commonly used task in MWP community. Therefore, we conduct very comprehensive experiments on three largest datasets, Ape-clean mentioned above, Math23k~\cite{wang2017deep} and MathQA \cite{amini2019mathqa}. We report the experimental results evaluated in answer accuracy. For the implementation of our solver, we connect PLM encoder with a tree-based decoder \cite{xie2019goal} to generate solutions, as shown in Figure \ref{fig:network}.
%At the beginning, we initialize the root node of the solution tree with the mean vector $\overline{Z} \in \mathbb{R}^{h}$ of the encoder output $Z$. The training process of encoder-decoder solver fine-tunes the pre-trained BERT encoder to understand well the given problem description and matches it a powerful decoder to translate the text into the correct equation. 
%We firstly transfer the generated equation tree into a value, then compare it with the ground truth value. The reported accuracy is the percentage of the correctly answered problems in the testing set.The comparison is based on how accurate the answer value is, rather than the equation. This is because one MWP can have multiple correct answer equations, which all lead to the same correct answer value. 

\input{table/tab_mwp_result}

\paragraph{Model Comparison.}
We first compare our approach with the most recent representative baselines on the benchmark Math23k dataset. The first baseline is \textsl{DNS} which is the pioneering work using the Seq2Seq model to solve MWPs. \textsl{Math-EN} \cite{wang2018translating} proposes an equation-normalization method and uses vanilla Seq2Seq model to get solutions. \textsl{S-Aligned} \cite{DBLP:conf/naacl/Chiang2019} applies a stack to generate target equations. \textsl{T-RNN} \cite{wang2019template} develops a template-based method with recurrent neural network. \textsl{GROUP-ATT} \cite{li2019modeling} is inspired by Transformer and implements a multi-head attention mechanism. \textsl{GTS} \cite{xie2019goal} proposes a goal-driven tree-based decoder and achieves great results. \textsl{KA-S2T} \cite{wu2020knowledge} proposes a novel knowledge-aware model that can incorporate background knowledge. However, their background knowledge still cannot bring external constants to equation generation, which means this model still struggles to solve difficult MWPs with external constants. \textsl{NS-Solver} \cite{qin2021neural} designs several auxiliary tasks to help training. \textsl{Graph2Tree} \cite{zhang2020graph} constructs two graphs during data pre-processing to extract extra relationships from text descriptions. \textsl{Multi-ED} \cite{shen2020solving} proposes a multi-encoder multi-decoder structure and achieves the best results on Math23K before our approach. \textsl{NumS2T} \cite{wu2021math} is the latest approach which uses explicit numerical values instead of number mapping to encode quantities. To avoid the implementation error that may cause unreproducible results of baseline models, we reported the results of these baselines from the papers where they were published, as many previous papers \cite{zhang2020graph,shen2020solving} did. For our method, we firstly report the results of vanilla BERT and RoBERTa, also with the performance of MWP-BERT and MWP-RoBERTa, which are pre-trained with our proposed tasks on Ape-210k and MathQA for Chinese and English evaluation.

For the English setting, we only report the results on most representative methods \textsl{GROUP-ATT} \cite{li2019modeling}, \textsl{GTS} \cite{xie2019goal}, and \textsl{Graph2Tree} \cite{zhang2020graph} following \cite{li2021seeking}. Because most baseline methods mentioned above are designed for the Chinese dataset.

The results in Table \ref{tab:main_result}  show that our approaches outperform previous methods by a large margin on both 2 datasets. Moreover, the BERT encoder with pre-training can further improve the accuracy. 

\begin{table}
\renewcommand\arraystretch{1.05}
\centering
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{|c|c|c|}
\hline
            & Math23k & Ape-clean    \\
\hline
DNS         & $50.3$  & $66.2$       \\
GTS         & $81.4$ & $73.2$        \\
\hline
RoBERTa  & $88.8$ & $80.2$  \\
BERT & $89.4$ & $80.4$  \\
MWP-RoBERTa  & ${90.2}$ & ${80.8}$ \\
MWP-BERT & $\mathbf{91.2}$ & $\mathbf{81.3}$  \\
\hline
\end{tabular}}
\caption{Comparison of answer accuracy (\%) between our proposed models and   baselines when they are all trained by the combination of the training set from Ape-clean and Math23k dataset. {Math23k} column shows the results when evaluating on the public test set of Math23k. Ape-clean column shows the result on Ape-clean test set.}
\label{tab:result_ape}
\end{table}


\paragraph{Evaluation on Ape-clean and Math23k  when Training by a Joint MWP Set.}

Since  Ape-clean is five times larger than Math23k, we are interested to evaluate whether MWP solvers trained on the Ape-clean dataset can perform well on the simple problems in the Math23k testing set. 
We combine the training set of Math23k and Ape-clean to train  the MWP-BERT model, and then measure the accuracy on the testing set of Math23k and Ape-clean separately. Results shown in Table \ref{tab:result_ape} convey interesting evaluation observations. Surprisingly, 
the accuracy of our models on Math23k reaches above 90\%, which is marvelously high (previous state-of-the-art methods can hardly reach 80\% \cite{shen2020solving}). 
Comparing to the results in Table \ref{tab:main_result}, even \textsl{GTS} has a higher accuracy when trained  with the big joint MWP set of Ape-clean and Math23k.
We can thus confirm that our curated Ape-clean dataset is able to serve as a high-quality MWP training set to improve  solvers'  generalization ability to solve problems in Math23k. 

\begin{table}
\renewcommand\arraystretch{1.05}
\centering
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{|c|c|}
\hline
 Model           & Accuracy    \\
\hline
QT(S)         & $87.3$      \\
QT(R)         & $88.7$    \\
QT(fix)      & $87.7$    \\
QT           & $90.8$    \\
\hline
BERT & $84.5$   \\
RoBERTa  & $84.6$ \\
MWP-BERT & ${91.0}$ \\
MWP-RoBERTa  & $\mathbf{91.5}$ \\
\hline
\end{tabular}}
\caption{Comparison of tagging accuracy (\%) between our proposed models and   baselines.}
\label{tab:result_tagging}
\end{table}

Moreover, the accuracy on Ape-clean of our approach is also much higher than other baselines (8\% higher than the strongest baseline \textsl{GTS}). Note that not all the baseline methods in Table \ref{tab:main_result} are presented in the comparison in Table \ref{tab:result_ape} for several reasons. First,  baselines like \textsl{Graph2Tree} and \textsl{Multi-ED} require specific data pre-processing like semantic parsing and POS tagging on new datasets. It is thus  hard for us to run them on the new Ape-clean dataset. 
Second, the experimental results in Table \ref{tab:main_result} have already shown the superiority of our approach over all other baselines. Last, \textsl{GTS} is widely acknowledged as a strong baseline for MWP solving and all following studies like \textsl{Graph2Tree}, \textsl{KA-S2T} and \textsl{Multi-ED} are based on \textsl{GTS}. %The performance of \textsl{GTS} in Table \ref{tab:result_ape} implies that \textsl{Graph2Tree} and \textsl{Multi-ED} will benefit as well from the Ape-clean dataset.  
We will leave the evaluation confirmation to the community by releasing Ape-clean soon.
%We also found that our improvement over \textsl{GTS} in terms of accuracy is significant by using t-paired test at 0.01 level.



\subsection{Quantity Tagging}
Quantity tagging \cite{DBLP:conf/acl/ZouL19} is firstly proposed to solve MWP examples with only addition and subtraction operators in their solutions. Briefly speaking, this task requires the model to assign ``+'', ``-'' or ``None'' for every quantity in the problem description and can serve as an MWP understanding evaluation tool to examine the model's understanding of each variable's logic role in the reasoning flow.  More exactly, this is also a classification task with 3 possible targets. We extract the corresponding vectors of all quantities according to their positions in encoded problem $Z$ from Equation \ref{encoder}. Next, a 2-layer feed-forward block is connected to output the final prediction. 

Following the setting in baseline method \textsl{QT} \cite{DBLP:conf/acl/ZouL19}, we perform 3-fold cross-validation and the results are given in Table \ref{tab:result_tagging}, which shows that PLMs benefits from the proposed mathematical pre-training and outperforms the baselines.


\subsection{Ablation Study}
We pre-train our BERT encoder with different settings and investigate the impact of each pre-training task on MWP solving model. As Table \ref{tab:data_ab} shows, self-, weakly- and fully- supervised pre-training are all able to improve MWP solving ability individually, and all sub-tasks do make contributions.  


\begin{table}[t]
\renewcommand\arraystretch{1.15}
\centering
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{|p{3.7cm}|m{1.6cm}<{\centering}|m{1.6cm}<{\centering}|}
\hline
    & Math23k & Ape-clean \\
    \hline
BERT & $89.4$ & $80.4$ \\
\hline
Only self-supervised & $90.4$ & $80.9$ \\
\quad  w/o MLM & $90.1$ & $80.6$ \\
\quad w/o $L_{s1}$ & $89.9$ & $80.5$ \\
\quad w/o $L_{s2}$ & $90.1$ & $80.4$ \\
\hline
Only weakly-supervised & $90.1$ & $80.8$ \\
\quad w/o $L_{w1}$ & $89.7$ & $80.2$ \\
\quad w/o $L_{w2}$ & $89.7$ & $80.4$ \\
\quad w/o $L_{w3}$ & $89.6$ & $80.5$ \\
\hline
Only fully-supervised & $91.0$ & $80.5$ \\
\quad w/o $L_{f1}$ & $90.5$ & $80.3$ \\
\quad w/o $L_{f2}$ & $90.6$ & $80.5$ \\
\hline
MWP-BERT & $\mathbf{91.2}$ & $\mathbf{81.3}$ \\
\hline
\end{tabular}}
\caption{The experimental results show the effectiveness of every pre-trained task. ``Only self-supervised'' means we only apply self-supervised pre-training on the BERT encoder. We also investigate the influence of each task. For example, ``w/o MLM'' means that we discard the MLM pre-training task and perform self-supervised pre-training. }
\label{tab:data_ab}
\end{table}


\iffalse
\subsubsection{Ablation Study on Pre-trained Model}
To evaluate the generalization ability of our pre-trained tasks and the MWP-BERT architecture, we also conduct the experiments that change the backbone encoder from BERT to RoBERTa \cite{liu2019roberta}. As Table \ref{tab:result_rbt} shows, the RoBERTa encoder can also benefit from our proposed pre-training tasks and achieve pleasant accuracy in terms of MWP solving on both Math23k and Ape-clean datasets. 

\begin{table}[t]
\renewcommand\arraystretch{1.2}
\centering
\setlength{\tabcolsep}{1.0mm}{
\begin{tabular}{|c|c|c|}
\hline
            & Math23k & Ape-clean    \\
\hline
RoBERTa w/o PT & $88.8$ & $80.2$ \\
RoBERTa w self PT & $89.2$ & $80.6$ \\
RoBERTa w weak PT & $89.3$ & $80.5$ \\
RoBERTa w full PT & $89.8$ & $80.3$ \\
RoBERTa w all PT & $\mathbf{90.2}$ & $\mathbf{80.8}$ \\
\hline
\end{tabular}}
\caption{Ablation study on RoBERTa. ``PT'' stands for pre-training.}
\label{tab:result_rbt}
\end{table}

\fi

==> text/old_introduction.tex <==
\section{Introduction}

%[BERT is strong. Understanding ability, multi-modal input, symbolic understanding BERT]
Pre-trained language models (PLM), like BERT~\cite{devlin2019bert} and RoBERTa~\cite{liu2019roberta}, have driven dramatic improvement in various natural language understanding tasks. PLM pipeline usually contains two key components: 1). pre-training on large scale corpus with self-supervised learning objectives to get contextualized representation; 2). fine-tuning on the specific downstream tasks. Great success in natural language understanding achieved by PLM also triggers widely usage of them in a large variety of tasks and applications in other fields, like twitter text \cite{qudar2020tweetBERT}, scientific text \cite{beltagy2019sciBERT}, biomedical data \cite{yoon2019pre,lee2020bioBERT}, and financial communications \cite{yang2020finBERT}. There are two major advantages of PLM techniques. The first one is that PLM can effectively make use of text examples in the self-supervised or weakly-supervised manner. The carefully designed pre-training tasks unlock the potential of large PLM in fully utilizing large text corpus, which is easy to collect. Secondly, the PLM style context encoding module can be easily plugged into various downstream tasks and consistently achieve great performance across various tasks. 
%cross-modal understanding works considering PLM paradigm, like CodeBERT for text-code understanding, Unicoder-VL for text-image understanding and HERO for text-video understanding. These cross-modal understanding tasks usually ask for learning effective representations of the same semantics under different modalities. These new representations are expected to boost the state-of-the-art performance across various downstream tasks.

\input{figure/fig_intro}

\textbf{Issues.} In this work, we aim at enhancing PLM with more effective numerical information capturing ability in a specific domain, math word problem (MWP) \textcolor{black}{understanding and} solving. Except for common contextual linguistic characteristics, MWP differs in two key parts: numerical value information and complex reasoning logic hidden in the context. As shown in Fig.~\ref{fig:intro}, perturbations in context content actually bring large variations in reasoning logic and equation. There are several issues if   
applying existing PLM in MWP solving. 
\begin{itemize}
    \item Most of PLMs do not consider built-in mathematical knowledge and are usually inefficient in capturing numeracy properties~\cite{DBLP:conf/emnlp/WallaceWLSG19}. Some works have proposed to inject numerical reasoning skill into PLMs via data augmentation~\cite{DBLP:conf/acl/GevaGB20} and designing different tokenization strategies~\cite{DBLP:conf/emnlp/0001RTER20}. Here, we aim at solving this issue by thoroughly exploring numeracy related pre-training objectives in MWP solving, which is orthogonal to previous study.
    \item Compared with pure numeracy embedding studies, MWP understanding and solving will suffer from the discrepancy between numeracy understanding (encoding) and solution generation (decoding). Injecting numeracy inductive bias in both encoding and decoding results in extra needs of Question-Solution parallel corpus. Single  contextual modeling does not consider this issue and will prevent broader application in various MWP data sources. In other words, we should keep PLM compatible with both examples with and without equation solutions so that the model can make use of more available data.
\end{itemize}
%Our goal is to design pre-training strategies in MWP understanding and solving tasks. Therefore, 
%Since most MWP solver regards number as tokens, the prominent information in these tokens can only be recognized by their context. Therefore, whether the model is able to grab this kind of number-related information in the context plays an important role in making correct reasoning. 
%However, existing PLM works give little concern about effectively incorporating this kind of number-related context information in the pre-training stage. Also, reasoning flows shown in equation trees can provide useful information, which would benefit MWP understanding. High-level reasoning ability keeps as an issue in PLM and equation tree can provide a way to understand how reasoning happens in this specific MWP solving task by leveraging dependencies between different sectors. At last, not all MWP examples are annotated with effective equation solutions.


%In order to address these issues, we conduct various studies on how to improve PLM paradigms by fully utilizing reasoning flow existed in complex equations as well as preserving numerical value information. 
Therefore, we present a suite of numeracy-augmented pre-training tasks with consideration of reasoning logic and get MWP-BERT for MWP understanding and solving. 
More exactly, we introduce several novel pre-training tasks with access to different levels of supervision signals. 
\begin{enumerate}
    \item Basically, one important part of pre-training tasks is designed for the self-supervised setting. 
Except for masked language modeling (MLM), we give extra consideration to number-related context information by designing related objectives. 
    \item Another part of pre-training objectives is about weakly-supervised setting (with answer annotations while without equation solutions). 
With access to the answer, we introduce several tasks to determine the type and the value of the answer. 
    \item The final part is about fully-supervised setting, where both solution equation and answer are available here. 
We propose to utilize equation structure in the training objective so that the PLM model is aware of the reasoning flow hidden in equation. 
We extend it by introducing different training objectives to incorporate reasoning flow in equations and numerical value information. 

\end{enumerate}

Moreover, in order to demonstrate the efficacy of our methods and support PLM training paradigm in MWP, we divided the dataset Ape210k \footnote{\url{https://github.com/Chenny0808/ape210k}} into two subsets. The former part named Ape-clean contains all solvable MWPs with equation annotations, which can be applied for fully supervised pre-training and also serve as a new MWP solving benchmark. The latter part consists of unsolvable MWPs and value-annotated (incompletely labeled) MWPs. Although these MWPs cannot be used to directly train a solver, they can serve on self-supervised and weakly-supervised pre-training tasks in the pre-training stage of MWP-BERT.

%Math word problem (MWP) usually refers to a textual description of a mathematical problem, which contains several known variables and asks for the answer of an unknown variable when solving it. More exactly, \textcolor{red}{as shown in Table \ref{tab:data_intro}}, MWP solving requires the generation of an equation showing how to get that unknown quantity. Not only accurate language understanding, but also strong mathematical reasoning ability is necessary in MWP solving. An expected MWP solver should be able to generate an equation which can exactly reach the answer value.


%Along the path of MWP solver development, the pioneer studies use traditional rule-based methods, machine learning methods and statistical methods \cite{yuhui2010frame,kushman2014learning,shi2015automatically,koncel2015parsing}, which are limited on two aspects. %However, they have two major drawbacks. Firstly, 
%Firstly, some of them rely on well-designed hand-crafted features, and are thus not efficient at all. Secondly, those solvers usually follow a template-based way to get answers and have poor generalization ability, since  they can only solve problems with given  answer templates. Afterwards, inspired by the development of sequence-to-sequence (Seq2Seq) models, MWP solving has been formulated as a pipeline of translating language descriptions to mathematical equations with neural network based encoder-decoder framework \cite{wang2018translating,wang2019template,DBLP:conf/naacl/Chiang2019,liu2019tree,li2019modeling,xie2019goal,zhang2020graph,shen2020solving}.



%Although those neural based models have achieved better performance than traditional methods, the best model on Math23k benchmark dataset until now \cite{shen2020solving} still sets gated recurrent units (GRUs) \cite{cho2014learning} as the backbone to perform text understanding task and encode input tokens. As is shown on recent studies of natural language understanding, pre-trained language models such as BERT (Bidirectional Encoder Representations from Transformers) \cite{devlin2019BERT} can perform perfect natural language understanding. It has been widely used in a large variety of NLP tasks and applications in other fields, like twitter text \cite{qudar2020tweetBERT}, scientific text \cite{beltagy2019sciBERT}, biomedical data \cite{yoon2019pre,lee2020bioBERT}, and financial communications \cite{yang2020finBERT}. There are two major advantages of BERT. The first one is that it is pre-trained with enormous language data without complex annotations. Those pre-training tasks enable a language model learning from non-annotated textual data, which is much easier to get than well-annotated data. Secondly, the BERT model can be plugged into various downstream tasks and achieve great performance than conventional language models. 

%Therefore, in this work, we proposed an MWP solver called MWP-BERT, which is composed of a BERT-based encoder and a tree-based decoder. To address the limits of BERT trained with free-form text on understanding mathematical text expression, we design several novel pre-training tasks, performing effective MWP-based pre-training. Moreover, we divided the dataset Ape210k \footnote{\url{https://github.com/Chenny0808/ape210k}} into two subsets. The former part named Ape-clean contains all solvable MWPs with equation annotations, which can be applied for fully supervised pre-training and also serve as a new MWP solving benchmark. The latter part consists of unsolvable MWPs and value-annotated MWPs. Although these MWPs  cannot be used to directly train a solver, they can serve on unsupervised and weakly supervised pre-training tasks in the pre-training stage of MWP-BERT. To the best of our knowledge, this is the first attempt in applying a pre-trained language model as a problem encoder to solve MWPs.


To sum up,  firstly, we propose a novel MWP-BERT, which is the first PLM model leveraging both numerical value information and reasoning flow in the equation to learn MWP representations. Secondly, in order to enable MWP-BERT's compatibility in making use of various kinds of training data, we design a hybrid schema in the pre-training stage, which contains self-, weakly- and fully supervised settings.
%\item We curate two new datasets, Ape-clean and Ape-unsolvable. Ape-clean contains around 100K samples with access to answer and equation solution for each example. It can support studies such as MWP model pre-training, MWP training dataset enlarging, and MWP solving. Ape-unsolvable contains about 120K samples with only  answers but no equations. It can be used for pre-training in self-supervised and weakly-supervised settings. 
Most importantly, MWP-BERT provides significant improvements on MWP solving, and achieves an accuracy above 90\% on Math23k dataset where the state-of-the-art baselines are below 80\%. To our knowledge, this is the first approach that surpasses human performance \cite{wang2019template} in terms of MWP solving.

%Firstly,  Secondly, in order to solve problems that need common-sense knowledge, we propose a keyword-based method to inject them into models. This can readily be used alongside any future improvements in pre-trained style MWP models. Thirdly,  Finally, experimental results on both Ape-clean and Math23k dataset show that our MWP-BERT achieves 5-10\% higher accuracy than previous baselines.
